Interpretable by Design: Learning Predictors by Composing Interpretable Queries

There is a growing concern about typically opaque decision-making with high-performance machine learning algorithms. Providing an explanation of the reasoning process in domain-specific terms can be crucial for adoption in risk-sensitive domains such as healthcare. We argue that machine learning algorithms should be interpretable by design and that the language in which these interpretations are expressed should be domain- and task-dependent. Consequently, we base our model's prediction on a family of user-defined and task-specific binary functions of the data, each having a clear interpretation to the end-user. We then minimize the expected number of queries needed for accurate prediction on any given input. As the solution is generally intractable, following prior work, we choose the queries sequentially based on information gain. However, in contrast to previous work, we need not assume the queries are conditionally independent. Instead, we leverage a stochastic generative model (VAE) and an MCMC algorithm (Unadjusted Langevin) to select the most informative query about the input based on previous query-answers. This enables the online determination of a query chain of whatever depth is required to resolve prediction ambiguities. Finally, experiments on vision and NLP tasks demonstrate the efficacy of our approach and its superiority over post-hoc explanations.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> connection_to_info_theory.tex <==
% !TEX root = TPAMI_IP.tex
If we take $Q$ to be the set of all possible binary functions of $X$, denoted as $Q_{\textrm{all}}$, then several information-theoretic quantities can be related to our framework. $Q_{\textrm{all}}$ is however \textit{not an interpretable query set} since most of the queries will be arbitrary subsets of $\gX$ without any clear interpretation/meaning (See Figure \ref{Fig: non-interpretable query set}b for an example). Nevertheless, these connections to coding theory could inspire follow-up works in developing more efficient algorithms for computing the optimal explanation strategy. These algorithms could in turn be used to compute hard-to-estimate quantities like mutual information and the Information Bottleneck \cite{tishby2000information} which have been extremely influential in representation learning \cite{hjelm2018learning, wu2020graph,gu2022self}. We present these connections in the following two propositions. Throughout this section, $\pi^*$ refers to the solution of \eqref{eq: complexity definition}.

%\myparagraph{Connections to Shannon's Information Measures.}
\begin{proposition}[\bf Connections with Mutual Information]
If $Q = Q_{\textrm{all}}$ and $expl^{\pi^*}_{Q_{\textrm{all}}}(X)$ is discrete, then
\begin{equation}
    I(X; Y) \leq H^{0}_{Q_{\textrm{all}}}(X; Y) - H(expl^{\pi^*}_{Q_{\textrm{all}}}(X)\!\! \mid\!\! Y) < I(X; Y) +  1,
    \label{eq: connection with MI} 
\end{equation}
where $I(X; Y)$ is the mutual information between $X$ and $Y$, and $H(expl^{\pi^*}_{Q_{\textrm{all}}}(X) \mid Y)$ is the conditional entropy of the explanation $expl^{\pi^*}_{Q_{\textrm{all}}}(X)$ given~$Y$.  Recall, $H^{0}_{Q_{\textrm{all}}}(X; Y)$ is the minimal expected description length when $\epsilon = 0$ in \eqref{eq: complexity definition}.
\label{proposition: MI and explainable entropy}
\end{proposition}

See Appendix \ref{Appendix: Connection with Shannon's Information Measures} for the proof. A corollary to the above proposition is that when $Y$ is a function of $X$ (which is often the case in supervised learning), then \eqref{eq: connection with MI} reduces to 
\begin{equation}
H(Y) \leq H^{0}_{Q_{\textrm{all}}}(X; Y) < H(Y) + 1,  
\end{equation}
where $H(Y)$ is the entropy of $Y$.\rene{A comment about the result and connection with prior art is missing.}

%\myparagraph{Connections to the Information Bottleneck}

The proposed framework is also related to the Information Bottleneck (IB) principle, which generalizes the notion of a minimal sufficient statistic. The IB seeks to compute a compressed stochastic representation $\tilde{X}$ of data $X$ such that a \textit{degree} of information is maintained about a relevant variable (or in our terminology the hypothesis) $Y$. This principle is encapsulated by the following optimization objective: 
%
\begin{equation}
\begin{aligned} 
\min_{\tilde{X}} I(X;\tilde{X}) - \beta I(\tilde{X}; Y) ,
    \end{aligned}
    \label{eq. IB principle}  
\end{equation}
or equivalently
\begin{equation}
\min_{\tilde{X}} I(X;\tilde{X}) \; \text{s.t.} \; I(\tilde{X}; Y) \geq \gamma,
\end{equation}

\begin{proposition}[\bf Connections with Information Bottleneck]
Given $Q = Q_{\textrm{all}}$ and $\epsilon=0$, if $expl^{\pi^*}_{Q_{\textrm{all}}}(X)$ is discrete, then $expl^{\pi^*}_{Q_{\textrm{all}}}(X)$ is a solution to the IB objective in \eqref{eq. IB principle} when $\beta \rightarrow \infty$ or equivalently $\gamma = I(X; Y)$. 
\end{proposition}

See Appendix \ref{Appendix: Connetions with Information Bottleneck} for the proof. It will be interesting to see if the computational framework developed in this paper can be utilized to develop new algorithms for computing the IB more efficiently than the current state-of-the-art. 


% We begin by showing some interesting connections between our work and Shannon's entropy, mutual information and the information bottleneck all of which require the special case in which the user selects $Q$ to be the set of all possible binary functions of $X$. Such a query set will however not be interpretable since majority of them will be arbitrary subsets of $\gX$ without any clear interpretation/meaning. We finally conclude by providing some approximation guarantees for IP. 


% \subsection{Connections to information theory}
% To understand the connections between our work and classical notions of information such as entropy, we revisit \eqref{eq: complexity definition} with $\epsilon = 0$, this corresponds to the scenario in which we want to solve the task ``exactly". This might be infeasible and often undesirable in practice. Nevertheless, we will consider this case for the purpose of analysis in this section. 

% Under any reasonable distance-like metric $d$, $\epsilon=0$ gives rise to the following optimization problem,
% \begin{align}\label{eq: complexity definition exact}
%     H_Q(X; Y) := &\min_{\pi} \E_{X}\left[|expl^{\pi}_Q(X)|\right]  \\
%     &\textrm{s.t.} \; p(y \mid x) = p(y \mid expl^{\pi}_Q(x)) \;\; \textit{(Sufficiency)} \nonumber \\
%     &\quad \forall (x, y) \in (\gX \times \gY) \nonumber
% \end{align}

% All our results in this subsection would be with regards to the above optimization problem.

% \myparagraph{Connection with Shannon's Information Measures} Entropy $H$ is often interpreted as the minimum number of yes/no questions needed on average to identify the state of a random signal $X$. Our measure, $H_Q$, is defined as the minimum number of ``interpretable" queries that need to be answered on average to infer a latent signal $Y$ from input $X$. $H_Q$ reduces (in spirit) to $H$ when we take $Q$ to be the set of all possible binary functions defined on $X$ and $Y$ is taken as $X$ itself, that is, the task is compression or reconstruction of the input signal. The key distinction here being that when $Q$ is taken to be all possible binary functions of $X$, most of them will not be interpretable to the user and thus the resulting ``explanation" would also be not interpretable. In this subsection we make this reduction concrete. 


% Given a query set $Q$, any feasible strategy $\pi$ partitions $\gX$ into the equivalence classes $[x]_{\pi, Q}$ defined in \eqref{eq: eq. class}. The recursive structure of $\pi$ along with the sufficiency constraint on the explanations generated by $\pi$ ensures that $\forall x' \in [x]_{\pi, Q}, \forall y \in \gY, p_{Y \mid X = x'}(y) = p_{Y \mid X = x}(y)$. 

% % Let the random function $\scrX^*_Q$ map each $x\in\gX$ to the index of the partition induced by the optimal strategy $E^*$.

% % Rigorously, $\scrX^*_Q(x) = \scrX^*_Q(x')$ iff $[x]_Q = [x']_Q$ $\forall x, x' \in \gX$.
% Before we present our main result, we note the following lemma.
% \begin{lemma}
% If $Q$ is the set of all possible binary functions of $X$ and $\pi^*$ is the solution to \eqref{eq: complexity definition exact} then $[x]_{\pi^*, Q} = \{x' \in \gX \mid p(y \mid x') = p(y \mid x) \; \forall y \in \gY\}$. 
% \label{lemma: eq.class when all binary questions}
% \end{lemma}
% That is, when $Q$ is unrestricted the optimal encoder induces a partitioning of $\gX$ such that $expl^{\pi^*}_Q(x) = expl^{\pi^*}_Q(x')$ iff $p_{Y \mid X=x}(y) = p_{Y \mid X=x'}(y')$ $\forall y \in \gY$. This leads to the following result relating $H_Q$ with mutual information.

% \begin{theorem}
% If $Q$ is the set of all possible binary functions of $X$ and $expl^{\pi^*}_Q(X)$ is takes finite number of values, then 
% \[  I(X; Y) \leq H_Q(X; Y) - H(expl^{\pi^*}_Q(X) \mid Y) < I(X; Y) +  1,\]
% where $I(X; Y)$ is the mutual information between $X$ and $Y$, and $H(expl^{\pi^*}_Q(X) \mid Y)$ is the conditional entropy of the explanation $expl^{\pi^*}_Q(X)$ given~$Y$.\!\!
% \label{theorem: MI and explainable entropy}
% \end{theorem}

% The proof is a simple application of Lemma \ref{lemma: eq.class when all binary questions}, Shannon's source coding theorem and the data-processing inequality with the insight that $expl^{\pi^*}_Q(X)$ is a sufficient statistic of $X$. A detailed proof is presented in Appendix \ref{Appendix: Connection with Shannon's Information Measures}. Theorem \ref{theorem: MI and explainable entropy} says that the \textit{$H_Q$ comes within 1 bit of the mutual information} modulo a residual conditional entropy term. We will now analyze the residual term for a few specific cases, 
% \begin{enumerate}
%     \item \textbf{Connections with entropy of $\boldsymbol{Y}$, $\boldsymbol{H(Y)}$}: If $Y$ is a function of $X$ and a discrete random variable, then we know $I(X; Y) = H(Y)$. In this case, $expl^{\pi^*}_Q(X)$ is a deterministic function of $Y$ since each equivalence class is the set of $x$ having the same label/hypothesis $y$ (in this case $p_{Y \mid X = x} = \delta_{Y(x)}$). Thus, $H(expl^{\pi^*}_Q(X) \mid Y) = 0$ and we obtain the following relation, 
%     \begin{equation}
%         H(Y) \leq H_Q(X; Y) < H(Y) + 1. 
%         \label{eq: entropy and complexity}
%     \end{equation}
    

%     \item \textbf{Connections with entropy of $\boldsymbol{X}$, $\boldsymbol{H(X)}$}: If the task is compression/reconstruction then $Y := X$ then $expl^{\pi^*}_Q(X)$ is a deterministic function of $X$. Now, if $X$ is discrete then we obtain the following relation
%     \[I(X; Y) \leq H_Q(X; Y) - H(X \mid Y) < I(X; Y) +  1 .\]
%      Adding $H(X \mid Y)$ to each term and using the relationship $I(X; Y) + H(X \mid Y) = H(X)$ we obtain
%     \[H(X) \leq H_Q(X; Y) < H(X) +  1.\]
% \end{enumerate}

% \myparagraph{Connection with the Information Bottleneck.} The Information Bottleneck (IB) principle generalizes the notion of a minimally sufficient statistic. It seeks to compute a compressed stochastic representation $\tilde{X}$ of data $X$ such that a ``degree" of information is maintained about a relevant variable (or in our terminology the hypothesis) $Y$. This principle is encapsulated by the following optimization objective: 
% \begin{equation}
% \begin{aligned} 
% \min_{p(\tilde{X}|X)} I(X;\tilde{X}) - \beta I(\tilde{X}; Y) ,
% %\sim &\min_{p(\tilde{X}|X)} I(X;\tilde{X}) \\ &\text{s.t.} \; I(\tilde{X}; Y) \geq \gamma
%     \end{aligned}
%     \label{eq. IB principle}  
% \end{equation}
% or equivalently
% \begin{equation}
% \min_{p(\tilde{X}|X)} I(X;\tilde{X}) \; \text{s.t.} \; I(\tilde{X}; Y) \geq \gamma,
% \end{equation}
% where the user-defined parameters $\beta$ or $\gamma$ control the trade-off between compression $I(X; \tilde{X})$ and sufficiency $I(\tilde{X}; Y)$. This principle has been heavily used in the deep learning literature to get efficient representations of data \cite{}, however the representation is an abstract random vector $\tilde{X}$ and is not constrained to be interpretable in any way. Indeed if we take the ``uninterpretable" query set as the set of all possible binary functions of $X$ then the $expl^{\pi^*}_Q(X)$ is a solution to the IB objective when $\beta \rightarrow \infty$. We state this formally in the following theorem. 

% \begin{theorem}
% If $Q$ is the set of all possible binary functions of $X$ and the random variable $expl^{\pi^*}_Q(X)$, where $\pi^*$ is the minimizer of \eqref{eq: complexity definition exact}, is discrete, then $expl^{\pi^*}_Q(X)$ is a solution to the IB objective in \eqref{eq. IB principle} when $\beta \rightarrow \infty$ or equivalently $\gamma = I(X; Y)$. 
% \end{theorem}


% Appendix \ref{Appendix: Connetions with Information Bottleneck} gives a detailed proof.

% \subsection{Approximation guarantees for Information Pursuit}
% \label{subsection: Approximation guarantees for Information Pursuit}
%  While in general it is difficult to have any performance guarantees for IP, in the case where $Q$ is the set of all possible binary functions of $X$, such that the entropy $H(q(X) \mid Y) = 0$ $\forall q \in Q$ and $Y$ is a function of $X$, we have the following proposition (see Appendix \ref{Appendix: proof of performance guarantee IP} for a proof). 
%  %Here $H$ refers to Shannon's entropy. 

% \begin{proposition}
% Let $Y$ be discrete. Let $\tilde{H}_Q(X; Y)$ be the expected description length obtained by the IP encoder. If there exists a function $f$ such that $Y = f(X)$ and $Q$ is the set to all possible binary functions of $X$ such that $H(q(X) \mid Y) = 0 \ \forall q \in Q$, then $H(Y) \leq \tilde{H}_Q(X; Y) \leq H(Y) + 1$.\!\!
% \label{proposition: Performance guarantee IP}
% \end{proposition}

% % While the above proposition is often considered to be true, this is the first time a rigorous proof has been presented (to the best of our knowledge). 
% Thus, in this special case, we have that $\tilde{H}_Q(X; Y) \leq H_Q(X; Y) + 1$ (using \eqref{eq: entropy and complexity}) and so the IP algorithm  provides a tight approximation to our proposed entropy measure. In the general case, the approximation guarantees of IP is still an open problem. We note in passing that when the query answers $q(x)$ are conditionally independent of each other given $Y$ and the number of queries that can be asked per input is fixed (as opposed to the variable length explanations, $|expl^{\pi}_Q(X)|$, proposed in \eqref{eq: complexity definition}) then it can been shown that IP achieves a near-optimal performance \cite{chen2015sequential}. In practice, we observe that IP manages to recover efficient (very small) explanations for different tasks (See Section \ref{section: Experiments}) even when these assumptions are violated. 


==> experiments_v1.tex <==
In the Introduction, we suggested four desired properties to guide the development of intepretable machine learning methods. \stewy{I planned the experiments section around these desired properties to give it some structure. Should we re-introduce these concepts in the intro for more coherence? Or would you rather I introduce and justify these desired properties in the experiments section, keeping them out of the introduction?}

\begin{enumerate}
    \item \textbf{Performance}: Does the method obtain competitive performance in comparison to non-interpretable models?
    \item \textbf{Domain-Intelligible}: For a particular task, are explanations of a form that can be understood by the user?
    \item \textbf{Minimality}: Are explanations succinct and of low complexity?
    \item \textbf{Faithfulness/Sufficiency}: In a statistical sense, do the explanations entirely explain the prediction?
\end{enumerate}

In this section, we quantitatively and qualitatively evaluate to what extent our method satisfies these desiderata across a range of tasks and query sets. 

Since our method's predictions are a function of the explanation, the explanation is a sufficient statistic for the prediction. So we satisfy faithfulness/sufficiency \textit{by construction}. Therefore we focus our evaluation on the other three properties. We perform experiments on vision datasets with two query sets: 1) image patches 2) human-friendly concept-based queries and on an NLP task with a third query set 3) the presence or absence of particular words.

\subsection{Tasks and Query Sets} \label{Section: Tasks and Query Sets}
\stewy{There is a lot to describe concerning the tasks + query sets as well as the baseline models we compare to in the following section. I will definitely cut the length down, but in this draft, I wanted to start with the longest and most detailed version.}

\myparagraph{Image Patch Queries} When we set queries to be the pixel values of image patches, we recover the familiar feature attribution-type explanations of post-hoc methods, although with a guarantee that the explanations are faithful. We apply this query set to the simple task of classifying binary images from MNIST (digit classification), KMNIST \cite{clanuwat2018deep} (Japanese character classification), and FashionMNIST \cite{xiao2017fashion} (clothing classification).

We set $Q$ to be the set of queries corresponding to all $3 \times 3$ overlapping patches in the image. All three datasets consist of images of size $28 \times 28$, so we have $26^2$ patches of size three, giving $Q = \{q_1, q_2, ..., q_{676}\}$. For any $q_i \in Q$, the answer $q_i(X) \in \{0, 1\}^9$ is simply the $9$ pixel values observed in image $X$ at the patch indexed by $i$. However, our factorization \eqref{eq: factorization of query answers} that we use to model $p(Q(x), z, y)$ no longer holds as the overlapping queries $q(X)$ are now \textit{causally related} (and therefore dependent even when conditioned on $Z$, making them unable to be modeled by a VAE). So instead we train a VAE to model the pixel distribution, and then compute the probability distribution over the patch query $p(q(x) | z, y)$ as the product of the probabilities of all pixels in that patch. See Appendix \ref{Appendix: Network architectures and training} for further training details.

\myparagraph{Concept-Based Queries} Now we consider a more complex classification problem with a concept-based query set. We use the Caltech-UCSD Birds-200-2011 (CUB) dataset \cite{wah2011caltech}, which contains 11,788 images of birds each belonging to one of 200 species. This fine-grained bird-species identification task typically requires domain expertise, but the concept-level explanations generated by our method make understanding the decision-making process accessible, even for a non-expert user.

Each image in the CUB dataset is annotated with 312 binary attributes representing high-level concepts in the image, such as the color and shape of the beak, wings, and head. However, these attribute labels are noisy, either because a part of the bird corresponding to that attribute is occluded or because they were simply labeled incorrectly. We follow \cite{koh2020concept} in deciding attribute labels by majority voting. For example, if more than 50\% of images in a class have black wings, then we set all images in that class to have black wings. It is natural to assume that birds in the same species will share the same attribute descriptions.

Our query set $Q$ consists of all 312 binary attributes. So as described in Section \ref{section: Information Pursuit}, we learn a VAE to model $p(Q(x), z, y)$, the distribution of concepts. However, we do not assume that images at test-time come with concept-level annotations $Q(x)$. So following \cite{koh2020concept}, we train a separate model $p_\theta(Q(x) | x)$, called a \textit{concept network}, that learns to predict the concepts $Q(x)$ in an image $x$. During inference for a particular image $x$, we use the concept network to answer the concept queries asked by IP. \textcolor{blue}{Missing some details here that will be provided by Aditya on sequential vs independent concept bottleneck stuff}

\myparagraph{Word-Level Queries} For NLP tasks, words make a natural first candidate for queries, being the fundamental semantic units of text. So for a vocabulary of words $V = \{ v_1, ..., v_n \}$, we consider queries $Q = \{q_{v_1}, ..., q_{v_n}\}$ where $q_{v_i}(x)$ is a boolean function determining if word $v_i$ is present in document $x$. We evaluate this query set on the Huffington Post News Category Dataset \cite{huffpostdataset}, a document classification task consisting of newspaper headlines and the corresponding categories they were published under in the Huffington Post newspaper. We stem all words in the dataset and choose the top-1,000 according to tf-idf score to be our vocabulary $V$.

\subsection{Models} \label{Section: Experiments.Models}
In Table \ref{fig: results table}, we compare our method with several other baselines intended to reflect the performance characteristics of our method.

The first two models in the table, \textsc{IP} and \textsc{Decision Tree}, seek minimal subsets of the query set to make predictions on, while the following two models, \textsc{VAE Posterior} and \textsc{Baseline on Q}, use the full query set. \textsc{Decision Tree} is a CART decision tree, with the information gain splitting criterion. While both methods form shallow decision trees that branch on responses to queries, the CART decision tree approximates mutual information gain from data while IP estimates it with a generative model, significantly improving performance in terms of both explanation length and final accuracy. See Appendix XX for more details on how stopping criterion $\epsilon$ was chosen for each model.

\textsc{VAE Posterior} uses the same generative model to make predictions as IP but has access to the full query set. For IP, we use ULA to sample from $p(z | s_k^{\pi_{IP}}(x), y)$, but now that we have access to the full query set $s_k^{\pi_{IP}}(x) = Q(x)$, we can improve performance by making use of the VAE's encoder instead. Following equation \ref{eq: marginalizing z}, we draw many samples from the encoder $p(z | Q(x), y)$ and then decode these samples to estimate the VAE's posterior distribution $p(y | Q(x))$. \textcolor{blue}{Appendix? For each problem, we set the number of samples to be the same as what we draw during each iteration of IP (12,000 for binary image tasks, 12,000 for CUB, 10,000 for HuffPost News). We call this model \textsc{VAE Posterior}}.

\textsc{Baseline} is a standard supervised neural network that receives $x$ as input. For MNIST, KMNIST, and FashionMNIST, \textsc{Baseline} is a convolutional network. For CUB, it is an MLP and for Huffpost News, it is an LSTM. Its counterpart \textsc{Baseline on $Q$} is also a supervised neural network but receives the full query set $Q(x)$ as input instead, illustrating the effect that using a particular query set has on performance. For MNIST, KMNIST, and FashionMNIST this is the same convolutional network as \textsc{Baseline} and for CUB and HuffPost News, it is an MLP. See Appendix XX for architectural and training details.

\begin{figure*}
\centering
\begingroup
\renewcommand{\arraystretch}{1.5} % Increase row separation - default value 1

\begin{tabular}{| l | c c | c c | c c | c c | c c |}
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{c}{MNIST} & \multicolumn{2}{c}{KMNIST} & \multicolumn{2}{c}{FashionMNIST} & \multicolumn{2}{c}{CUB Birds} & \multicolumn{2}{c}{HuffPost News} \\
 & Acc & $L$ & Acc & $L$ & Acc & $L$ & Acc & $L$ & Acc & $L$ \\
\hline
\textsc{IP} & 96.78\% & 5.16 & 91.02\% & 16.02 & 85.40\% & 18.10 & 76.37\% & 11.08 & 71.21\% & 199.36 \\
\textsc{Decision Tree} & 90.23\% & 12.16 & 78.00\% & 13.86 & 80.80\% & 9.02 & & & 63.00\% & 112.02 \\
\hline
\textsc{VAE Posterior} & 98.97\% & - & 94.25\% & - & 87.56\% & - & & & 71.72\% & - \\
\textsc{Baseline on $Q$} & 99.15\% & - & 95.10\% & - & 86.96\% & - & 75.70\% & - & 71.48\% & - \\
\hline
\textsc{Baseline} & 99.15\% & - & 95.10\% & - & 86.96\% & - & 82.70\% & - &   & - \\
\hline
\end{tabular}
\endgroup

\caption{Classification accuracies and explanation length $L = \E_X [|expl_Q^\pi(X)|]$ on a variety of methods and datasets. See Section \ref{Section: Experiments.Models} for more details on the models in the table. \stewy{Cells that are blank correspond to baselines that are not quite done yet. Dashes mean that the metric is not applicable to that particular method.}}
\label{fig: results table}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=0.4 \textwidth]{figs/Acc_Minimality_Plot.pdf}
    \caption{Accuracy vs. IP's Average Explanation Length as the mutual information stopping threshold $\epsilon$ varies. \stewy{Should be a plot of relative test accuracy instead}}
    \label{fig:accuracy_minimality_plot}
\end{figure}

\subsection{Performance and Minimality}
The performance of IP relative to traditional non-interpretable methods depends on three factors: 1) the sufficiency of the query set 2) the posterior accuracy of the generative model and 3) the value of the $\epsilon$ parameter governing the performance-minimality trade-off. We perform experiments to measure the relative impact of each of these factors across tasks and query sets. In this section, we also study the length of generated explanations and find that our method generates surprisingly short explanations...?

\myparagraph{1. Query Set Sufficiency} Since IP receives queries as input, it can only perform as well as the query set is sufficient for the task. In Table \ref{fig: results table}, we compare the performance of IP with other baselines, including standard non-interpretable models. We can get a sense of how nearly sufficient the query set $Q$ is for a task by comparing the accuracies of the non-interpretable \textsc{Baseline} (which has access to the full input $x$) with those of \textsc{Baseline on $Q$} (which only has access to query responses $Q(x)$).

In the case of image patch queries, the query set is trivially sufficient as it reconstructs the image itself. Therefore, the accuracies of \textsc{Baseline} and \textsc{Baseline on $Q$} are identical on the binary image classification datasets. On CUB and HuffPost News however, there is a sizable drop in accuracy when only the query set $Q(x)$ is observed. For HuffPost News, the query set is the presence/absence of words from a vocabulary of size 1,000. \stewy{Need to finish RNN text baseline experiment here:} So the query set loses ordering information, which causes a ... drop in accuracy .... For CUB, as mentioned in Section \ref{Section: Tasks and Query Sets}, we pre-process the attribute labels for each image in such a way that the class is known to be fully determined by these attributes. However, at test time, we do not have access to attribute labels, and estimate them from the raw image using a trained concept network. While this process leads to a decrease in performance between \textsc{Baseline} and \textsc{Baseline on $Q$}, it enables powerful, human-interpretable concept-level queries. Choosing the right query set for a task is non-trivial and affects both the quality of final explanations as well as the performance of the method. We cover further design considerations in \ref{Section: Domain Intelligibility}.

\myparagraph{2. Posterior Accuracy of the Generative Model} Another significant difference between our method and traditional approaches is that we use the posterior of a generative model to make predictions $p(y | s_{k}^{\pi_{IP}}(x))$. Therefore, the performance of the VAE's posterior $p(y | Q(x))$ given the full query set gives an upper bound to the performance of IP, which only has access to a portion of the queries. Table \ref{fig: results table} shows that the VAE's posterior accuracy is within 2\% of its standard supervised counterpart \textsc{Baseline on $Q$} across all problems tested, validating our approach of using the posterior of a conditional VAE as a predictive model.

\myparagraph{3. Accuracy-Minimality Tradeoff}
Finally, unlike standard supervised methods, we seek to use only a small subset of queries to make a prediction. IP terminates on a given input once a certain metric reaches a stopping threshold $\epsilon$. For the binary image tasks, we terminate once the probability of the most confident class exceeds 99\%, or equivalently once the remaining uncertainty in the prediction is less than 0.01. For CUB and HuffPost News, we terminate once the highest mutual information of any remaining query falls below a certain threshold (0.05 and $10^{-3}$ respectively).

As described in Section \ref{section: info theory connections}, this $\epsilon$ corresponds to how approximately sufficient the generated code is for task $Y$, thereby controlling an accuracy-minimality tradeoff. When $\epsilon$ is large, the stopping criteria is quickly reached, so IP produces short explanations, but with a loss in accuracy since there is high uncertainty in the model's predictions. When $\epsilon$ is small, the generated explanations are more nearly lossless codes for $Y$, but may be prohibitively long.

\stewy{Describe minimality plots here (Figure \ref{fig:accuracy_minimality_plot}) - still TODO}

\begin{figure*}
    \centering
    \begin{tabular}[]{c}%
        \subfloat[MNIST digit classification - Image Patch Queries]{
            \includegraphics[width=0.5 \textwidth]{figs/IP_in_action_MNIST.eps}
            \label{fig:IP MNIST in action}
        } \\
        \subfloat[CUB bird identification - Concept-level Queries]{
            \includegraphics[width=0.65 \textwidth]{figs/IP_in_action_CUB.eps}  \label{fig:IP CUB in action}
        }
    \end{tabular}
    \quad
    \subfloat[HuffPost News document classification - Word-level Queries]{
        \includegraphics[width=0.27\textwidth]{figs/IP_in_action_HuffPost.eps}
        \label{fig:IP Text in action}
    }%
    
\caption{Visualizations of IP's decision-making process across several tasks. In Figure \ref{fig:IP MNIST in action}, the top row displays the test image with red boxes denoting the current selected patch and blue boxes denoting previous patches. The second row shows the revealed portion of the image that the predictive model gets to use at each query. The final row shows the model's estimated posteriors at each query, beginning at a nearly uniform prior before converging on the true digit ``6'' after 4 queries. The left image in Figure \ref{fig:IP CUB in action} is the input image and on right we have a heatmap of the estimated class probabilities at each iteration. We only show the top 10 most probable classes out of the 200. To the right, we display the queries asked at each iteration, with red indicated a ``false'' response and green a ``true'' response. In Figure \ref{fig:IP Text in action}, we again show a heatmap of estimated class probabilities at each iteration. Words colored in red are absent from the sentence while words in green are present.}
\label{Fig: IP in action}
\end{figure*}

% \caption{IP MNIST in Action - \textit{Semantic coding of image $x^0$ using IP. Each column depicts specific snapshots of the state of the IP algorithm as the iterations proceed. We will now explain each row in detail. \textbf{(a)} Each column depicts parts of $x^0$ seen by IP in each iteration. These parts are highlighted by the overlayed $3 \times 3$ squares. The red square indicates the current queried patch while the blue squares indicate past queries. The number at the top-left corner indicates the iteration number $k$. \textbf{(b)} In each column we show the image content unveiled by IP corresponding to the queries chosen until that iteration. White or black indicate the image intensities at that pixel. The gray background illustrates the parts of the image that have not been queried till iteration. \textbf{(c)} Each column is a bar plot representing the posterior distribution $P(Y \mid B_{x^0, k})$, that is, the distribution over digit labels given the image intensities observed until iteration $k$.}}

\subsection{Domain Intelligibility} \label{Section: Domain Intelligibility}
\stewy{Need a short intro/topic sentence here to orient the reader. This subsection should probably also appear towards the beginning of the experiments section.} Figure \ref{fig:IP MNIST in action} illustrates a typical run of our algorithm on a test image from MNIST, choosing $3 \times 3$ patches until termination. The first query is near the center of the image; recall from \eqref{def. IP algorithm} that this choice is independent of the particular image and represents the patch whose pixel values have maximum mutual information with $Y$. After seeing a vertical white line through this center patch, the updated posterior concentrates its mass on ``1''. By the fourth query, the model expects the digit to be either a ``6'' or ``8''. The next query is well-suited to separating sixes and eights, being a patch in a region that should be black for an ``8'' but could contain a vertical white stroke for a ``6''. Upon discovering such a vertical stroke in that patch, the algorithm reaches high confidence in the image being a ``6'' and terminates. From Table \ref{fig: results table}, the average explanation length is only 5.16 queries. Paired with visualizations of the posteriors at each iteration, these patch explanations are concise and easy to interpret on MNIST digit classification.

However, Table \ref{fig: results table} shows that even slightly harder classification tasks like KMNIST and FashionMNIST require significantly more patch queries. Low-level patch queries are ill-suited to complex vision tasks, where they may be hard to interpret and lead to very long explanations.

In contrast, on the much more complex 200-class CUB bird identification task, IP with concept-level queries converges on the correct class after just 11.08 queries on average. Figure \ref{fig:IP CUB in action} shows IP's inference process. This example illustrates a common emergent query selection strategy. After converging on just four possible bird species out of the 200 by query 5, IP chooses queries that would verify/descredit specific classes among its highest probability predictions. Green Jays and Scott Orioles have black breasts, so they are ruled out after query 6. Likewise, Tropical Kingbirds are buff-colored (a yellow ochre) while Great Crested Flycatchers are brown. These concept queries lead to concise and easily-understood explanations, even on a fine-grained dataset that typically requires expert knowledge to perform accurate classification.

Lastly, in Figure \ref{fig:IP Text in action} we display an example run of IP on the HuffPost News Category Dataset. The query responses are much sparser, since each sentence only contains a few words out of the 1,000 in the vocabulary. As a result, most queries are not very informative, so IP requires more queries, 125 in total. However, due to the sequential nature of our algorithm, by plotting how the predicted class probabilities change with each query, we can gain insight into the prediction, even with a comparatively large number of queries. Upon reaching its first positive query ``eat'', the probability mass concentrates on the categories ``Food \& Drink'' and ``Wellness''. However, as the queries ``citi'', ``visit'', ``york'', and ``bar'' come back positive, the model becomes more and more confident that ``Travel'' is the correct class.

In general, we seek query sets that lead to concise, intelligible explanations that are also sufficient for the task. Choosing a good query set for a given problem is non-trivial and requires an understanding of the important structure in the data. In particular, concept-level queries are promising as an approach towards interpretable, concise, faithful explanations for complex machine learning tasks.

%\myparagraph{Semantic entropy across different datasets} We compute the semantic entropy of binary image classification on four different datasets: MNIST, FashionMNIST, KMNIST, and Caltech Silhouettes. Each entry $(i,j)$ of Table \ref{Fig: Results} indicates the semantic entropy computed for dataset $j$ such that the code is sufficient to predict the labels at accuracy level $i$. By tuning $\epsilon$ we compute $\tilde{SE}^{\epsilon}_Q(X; Y)$\footnote{The sub-optimal solution to $SE^{\epsilon}_Q(X; Y)$ computed by IP.} such that the label $Y$ is predicted with the desired accuracy level. In other words, we compute the minimum number of $3 \times 3$ patches that need to be revealed on average to predict the class label with a given degree of accuracy. To normalize for the effect of different datasets having different Bayes error rates, we used relative test accuracies which are the accuracies obtained by predicting $Y$ according to $\argmax_{y \in \gY} p(y \mid B_{x, L})$\footnote{Recall $L$ is the iteration after which IP terminates} divided by the prediction made upon observing the entire image (all the patches indexed by $Q$). Our findings indicate that MNIST $<$ FashionMNIST $<$ KMNIST $<$ Caltech Silhoettes in terms of semantic entropy at almost all relative test accuracy levels. For example, to obtain a relative accuracy of $0.95$ about 5 patches on MNIST need to be revealed on average, whereas for Caltech Silhouettes about 34 patches are required on average. Intuitively, this trend is expected since the amount of image variations is much higher in the Caltech dataset, which has about a hundred different object classes, than in the MNIST dataset. In Appendix \ref{Appendix: approximate continous plots for semantic entropy} we report more results highlighting the trade-off between accuracy level and semantic entropy. Interestingly, the ordering of MNIST $<$ Fashion-MNIST has been reported in prior work on task complexity in context of deep learning \cite{achille2019information}.

% \myparagraph{Most informative regions of an image} An advantage of using patches as queries is that it gives a natural measure of how information is distributed within an image. Since all the datasets considered have centered images, we can plot class-specific heatmaps. Each pixel in a class-specific heatmap represents the probability that this pixel would be part of the approximately minimal explanation computed by IP for a randomly chosen image from the same class. Heatmaps of selected classes from different datasets are provided in Figure \ref{Fig: semantic_examples}. Several interesting patterns emerge. For example, the heatmaps for both ``$3$" and ``$5$" indicate that most semantic codes for these classes concentrate on the top-right and top-left regions of the image where intuitively the distinguishing feature (curved head) lies. The only distinguishing feature in the Caltech dataset are object shapes and edges since it is comprised of silhouettes. The two examples provided of ``Airplane" and ``Motorbike" highlight this. Finally, the semantic codes for both ``T-Shirt" and ``Pullover" are concentrated near the arm regions since this is the most distinguishing feature between the two classes. Notice how the code almost never contains the internal region of the T-shirt/Pullover. Note, these heatmaps are a consequence of the semantic code computed by IP and are not to be confused with attribution maps commonly employed in literature to explain neural network decisions.


%\begin{table}[h]
%\centering
%\caption{\textit{Semantic Entropy of different datasets at varying levels of desired relative test accuracies. Each entry $(i,j)$ in the table indicates the semantic entropy computed for dataset $j$ such that the code is sufficient to predict the labels at accuracy level $i$.}} 
%\vspace{2mm}
%\includegraphics[scale=0.55]{figs/dataset_comparisons.png}
%\label{Fig: Results}
%\end{table}

%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.43]{figs/semantic_examples.png}

%\caption{\textit{Most informative regions in an image for a class. Each column corresponds to a class (written at the bottom). (\textbf{a}) Each row depicts the average image of the corresponding class computed from the training set. (\textbf{b}) Each column plots the corresponding class specific heatmap. Best viewed in colour.}} 
%\label{Fig: semantic_examples}
%\end{figure}

==> intro_0.tex <==
\IEEEPARstart{I}{n} recent years, 
``explainable" prediction has emerged as a major priority in machine
learning. This shift of focus is largely motivated by sensitivity to
risk and the desire, even necessity, for transparency in
decision-making, especially when decisions impact human lives.  In
such domains, understanding \textit{how} a decision is reached may be
as important as achieving high predictive accuracy.  For example, a
new ``computational algorithm'' for diagnosing a disease, predicting
its progression or response to treatment, cannot enter clinical
practice unless scientists and regulators can deconstruct the decision
rule in the domain language, i.e., in terms of the underlying biochemical mechanisms \stewy{Citation? If this is a general comment, then should be phrased more generally}.%\rene{Great example. Since we don't talk about this later in the paper, I wonder if we shouldn't have an example that is closer to the type of data we will have experiments on.}

\stewy{Could use transition, even a simple word like "However,"} It is widely believed that there exists a fundamental trade-off in machine learning between explainability and predictive performance. Shallow models like decision trees and linear classifiers are often considered very explainable but their accuracy is limited compared to deep neural networks. As a result, most attempts at explainability involve \textbf{\textit{post-hoc}} explanations for trained deep networks, supplementing network decisions with annotations and commentary thereby maintaining accuracy. %\rene{Sharp transition. The trade-off comes out of the blue. Moreover, the rest of the paragraph focuses exclusively in post-hoc, without connecting post-hoc with the tradeoff. One solution could be to move the tradeoff elsewhere and simply focus here on 'One of the most common approaches to interpretability involves post-hoc explanations. Another solution is to better explain the tradeoff: say that interpretability adds constraints to learning, which could result in suboptimal features, and reduce predictive accuracy.}  
For example, given an already trained black-box model, explain the output using attribution maps which estimate the contribution of individual features to the decision. Typically, these maps reflect the effect of perturbations of the input, for instance, gradients of the network output with respect to input features \cite{baehrens2010explain, simonyan2013deep} and are easily integrated with a pre-trained network %\stewy{Is it fair to say these typically involve perturbations of the input? LIME does, saliency maps could be thought of this way, but SHAP is harder to argue without unduly hiding complexity. Why not just introduce a couple methods explicity? E.g. Common approaches include saliency maps, where attributions correspond to gradients of the network output with respect to input features \cite{baehrens2010explain, simonyan2013deep} and those based on game-theoretic Shapley values, which make predictions on random subsets of the features to determine the importance of each feature (ADD CITATION HERE).}.  
Recent critical appraisals can be
found \cite{adebayo2018sanity, yang2019benchmarking,
	kindermans2019reliability, shah2021input, slack2020fooling};
see Section \ref{sec:related_work}.

% {\bf Integrate the next paragraph into Related Work.} 
% \textcolor{red}{However, these methods have
	% at least two major shortcommings.  One drawback is that the
	% explanations may not be faithful to the underlying model.  If a
	% post-hoc/attribution method generates a false explanation it is often
	% impossible to decipher if the explanatory method has failed or if the
	% model indeed made its prediction for the wrong reasons.  Perhaps the
	% most common pitfall of attribution methods is that in order to explain
	% why an algorithm predicts class $y_1$ instead of class $y_2$, it
	% highlights a particular region, and when it asked to do the same for
	% class $y_2$ it highlights the same region of the same image
	% \cite{rudin2019stop}. This is because attribution maps only tell what
	% part of the input is being used and not how it is used.}
Perhaps the most common pitfall of attribution methods is that in order to explain
why an algorithm predicts class $y_1$ instead of class $y_2$, it
highlights a particular region, and when it asked to do the same for
class $y_2$ it highlights the same region of the same image
\cite{rudin2019stop}. This is because attribution maps only tell what
part of the input is being used and not how it is used.
Indeed, this begs the question, what does interpretability mean and what are the ideal units of interpretability? Contributions of raw features/neurons towards the final prediction are usually not the most intuitive or interpretable explanations for humans \cite{koh2020concept}. Rather, the end-user might be more attuned to thinking about semantic concepts and associated high-level patterns in the data \cite{armstrong1983some,tenenbaum1999bayesian} or about causality and mechanism expressed in a procedural manner in 
technical domain-specific
language \stewy{This causality and mechanism phrase is a bit unclear to me. I get generally what it is saying, but not everything. I think it could be better just to leave this phrase out.}.

%There are of course many ways to define an ''interpretable'' decision;
%anything can be called an ''explanation.'' 
% but explanations are only \textit{useful} insofar as they constitute 
%\textit{evidence}

In this paper, ``explainable" entails a description
in words, symbols or patterns of the {\it reasoning} leading to the decision. For instance, in image classification, a model is often considered ``explainable" if its decision can be understood in terms of patterns occurring in salient parts of the image \cite{chen2019looks}. Some words or patterns may be domain-dependent and therefore not interpretable to non-experts. %\rene{I think we need to add one more case to accommodate something like: what regions of the image are most important for making this prediction? Otherwise, we risk the usual comment that what we do isn't all based on symbols and reasoning. We do not want to tell the reader this is a reasoning paper.} 
Hence explainable
evidently depends on the end user, namely the person who is trying to understand or ``deconstruct'' the decision taken by the algorithm. Two extreme cases are explanations entirely composed of ordinary words, e.g., in semantic scene interpretation, and explanations involving physio-chemical mechanisms and expressed entirely in mathematics. 

%Useful ''explanations'' are then inherently domain-
%dependent.  For instance, in image classification explanations in
% terms of different parts of the image might be acceptable
% \cite{chen2019looks}, whereas for medical diagnosis a practitioner
% might more interested in explanations in terms of key concepts like
% ``Is the space between knee joints too narrow?" for determining if the
% x-ray image shows osteoarthritis.
We observe that interpretable explanations are often compositional in that they are constructed from
elementary units, for instance, words, parts of an image, or domain-specific concepts. The explanation of the entire model depends on the interpretability of these elementary units. As a result, these elementary units ought to be user-defined according to the domain. We also argue that in order to be most interpretable, the explanation composed of these elementary units should be as concise as possible. For example, a boolean expression with ``interpretable" literals is only considered interpretable if the total number of literals is small enough to be parsed by a human. Finally, we would like this composition of elementary units, the explanation, to be a sufficient statistic of the model's prediction. This is important for complete transparency of the decsion-making process, since this implies that the model prediction will not be affected by aspects of the input not accounted for by the explanation.

% {\bf Integrate next paragraph into Related Work.}
% \textcolor{red}{Post-hoc interpretability methods are not of this nature.
	% Attention-based models are a popular family that are often considered
	% ``interpretable" \cite{de2019bias, galassi1902attention}. However,
	% attention is only a small part of the overall computation and can be
	% easily manipulated to hide model biases \cite{pruthi2019learning}. We
	% note in passing that there have been efforts to develop ML models that
	% are ''interpretable by design'' \cite{alvarez2018towards,
		% chen2019looks, nauta2021neural}. However the interpretable units are
	% learned from data, e.g., classifiers for common shapes, and may not
	% align with the key concepts identified by the user.}

% \begin{enumerate}
	%     \item \textbf{Sufficiency}: Explanations are sufficient statistics for model predictions.
	%     \item \textbf{Intelligibility}: Explanations are understandable to the end user.
	%     \item \textbf{Minimality}: Explanations are as short as possible while maintaining the other three properties.
	%     \item \textbf{Performance}: The overall method obtains competitive performance compared to black-box models.
	%     %\item (\textit{Counterfactual Power}:)? 
	% \end{enumerate}

% \textcolor{red}{Good points in this para, not sure where it fits}
% \textcolor{blue}{
	% Need to motivate our choice of desirable properties...
	% Sufficiency: Anything can be called an explanation, but explanations are only \textit{useful} insofar as they constitute \textit{evidence}. Let $z$ be an explanation for the model prediction $\hat{y} = \arg\max_y p(y|x)$. Then $z$ must increase $p(\hat{y} | z) > p(\hat{y})$ and decrease the probability $p(\text{not } \hat{y} | z) < p(\text{not } \hat{y})$. An explanation that has the power to can explain anything has no power at all. This property highlights a major issue with many post-hoc attribution methods. Perhaps the most common failure mode of saliency maps is that when asked to explain why the model predicted class $y_1$, it highlights a particular region, and when asked to explain why the model predicted class $y_2$, it highlights the same region of the same image.}\rene{Excellent point}

We address the subjective nature of explainability by allowing the user to specify a family $Q$ of task-specific functions of input
data $X$ called \emph{queries}, which are by construction
interpretable to the user. Possible choices for $Q$ include:

\begin{enumerate}
	\item \textbf{Small image patches:}
	The query simply asks to see the pixel intensities of a particular
	patch of image X. In this case, the number and locations of the
	patches that need to be revealed to solve a task give a natural
	measure of how the information content is distributed within an image.
	%These explanations are reminiscent of the attribution maps
	%generated by post-hoc interpretability methods. However, unlike these
	%methods, we want our generated explanations to satisfy properties $2$
	%and $3$ as well. 
	For example, we might want a method that provides the
	smallest set of patches that is sufficient for predicting $Y$, the class label.
	
	%our explanations are not post-hoc - they are causal. Furthermore, the recursive structure of our encoder allows for an additional layer of interpretability by analyzing the decision traceback which isn't possible in attribution methods \ref{Sec. Experiments}.
	
	\item \textbf{Concept-based explanations:}
	In domains such as medical diagnosis or species identification,
	the user might be interested in receiving explanations in terms of
	concepts identified by the community to be relevant for the task. For
	instance, is this bird a ``Crow" because of its beak shape, its feather
	colours or both? In our framework, by simply choosing a query for each of
	these concepts (feather colour/beak shape) the user can easily obtain such concept-based 
	explanations.
	
	\item 
	
	\textbf{Visual scene information:} In visual scene understanding, one seeks a rich semantic description $Y$ of a scene $X$ by accumulating
	the answers to queries about the existence of objects and
	relationships, perhaps generating a scene graph \cite{jahangiri2017information}. One can design a query set $Q$ by instantiating these queries with trained classifiers. The key insight is that while $|Q|$ may be large, due to context only a few queries might be sufficient to completely characterize the semantic content of the scene. 
	
	
	
	% For such use-cases, $Q$ could be the set of
	% all binary functions indicating the existence of entities,
	% their attributes or relationships with other entities, all relative
	% to some pre-specified vocabulary and some
	% designated region of the image $X$. For example, a particular query
	% could be 
	% ``Is there a person in the top left corner of the image?" and the
	% task could be to find the attributed graph which describes all
	% the semantic content of the scene in terms of
	% objects, their arrangements, attributes and relationships. The key
	% insight is that while $|Q|$ may be large, due to context only a few
	% queries might be sufficient accomplish the task, i.e., to completely 
	% characterize the semantic content of the scene as defined by $V$.
	% See ([],[],[]) and the literature on VQA.
	
	\item \textbf{Deep neuron-based explanations:} 
	The above three examples are query sets $Q$ based on domain knowledge. We
	could also design $Q$ for which each query corresponds to the
	activation level of a neuron in a trained deep network. Such a query
	set $Q$ is naturally learnt from data and sufficiently expressive at
	solving the task at hand\footnote{Owing to the representational power
		and expressiveness of modern deep networks.}. One could leverage
	recent techniques \cite{mu2020compositional, bau2017network,
		hernandez2022natural} to interpret the computations of each individual
	neuron in a network.
\end{enumerate}

At first glance, classical decision trees
([],[],[]) based on $Q$ might appear to do the job, in fact ``by
design.'' Here we are referring to standard tree induction from
labeled training data where the assignment of queries to internal nodes is driven by stepwise uncertainty reduction. The reasoning behind the decision is then largely transparent, expressed by the sequence of queries and their answers encountered along the path from
root to leaf determined by the data. Indeed, this is why decision trees are often favored in applications such as medical diagnosis, where the queries are based on the outcome of lab tests and clinical examination.

However, the accuracy is usually inferior to state-of-the-art methods
in machine learning;%\rene{I think here the point of the trade-off between interpretability and accuracy is made much more clearly and with more context than at the beginning.} 
one simply cannot pose enough queries to achieve
a competitive error rate, at least in complex high-dimensional prediction, even with gigantic amounts of labeled data, due to data fragmentation. Moreover, it is not feasible to even store an entire tree of significant depth. Whereas random forests ([],[]) ameliorate
the depth issue (since many more features can be exploited) and are often much more competitive in accuracy, they sacrifice interpretability, the very property we want to hardwire into our decision algorithm. One way to maintain both the interpretability of a single tree and the accuracy of a forest of trees %\stewy{Random forests can be ok, but certainly don't compare to deep models on certain kinds of tasks. That's not really the baseline we care about. What if instead, we kept the comparison to uninterpretable deep networks?}
, is a model-based construction
([],[]) based on the joint probability distribution of $(Y,Q(X))$, where
$Y$ is the target variable. To our knowledge, this approach has not been successfully implemented, probably due to two
liabilities. The first one is the size of the data structure if dozens of queries are required for good performance; we cannot learn and
store a tree of depth on the order of 100. The second problem is that
the only feasible models to date assume the queries %, which must be answered with trained classifiers, 
are conditionally independent given $Y$. But
this degrades performance in practice [] due to the complex dependency structure in real data.

We propose to overcome these issues as follows: First, in any actual instance of prediction, the data are fixed, e.g., an image to be annotated with respect to queries. Consequently, for that instance, say $x^{obs}$, we do not need the entire tree; we only need
the branch traversed by the queries in $Q(x^{obs})$, which can be determined online - at the time of prediction ([],[],[]). Second, the
emergence of powerful new generative models based on deep learning, such as variational autoencoders (VAEs), enable a model-based approach in which the queries are decoupled by introducing latent variables, thereby rendering feasible the optimization of query selection with Monte Carlo sampling. \stewy{This and paragraph before are slightly confusing to the new reader - could be tighter.}

In this paper we make the following contributions,%\stewy{I think a contribution list is generally a bit more compact. Each bullet point is usually one sentence, sometimes two. However, there is also a lot of good stuff in here that the user would want to know.}
\begin{itemize}
	\item We present a novel framework for prediction in machine learning which
	is explainable by design. We allow the end-user to specify a query set
	$Q$ and then formulate learning as an optimization problem over strategies that
	minimizes the number of queries needed on average to predict $Y$ from
	$X$, assuming $Q$ is a sufficient statistic for $Y$. 
	\item This \textit{minimum number of queries needed} generalizes the notion of Shannon's entropy which is obtained (within 1 query) when $Q$ is taken to be the set of all possible binary functions (all of which are not necessarily interpretable). We explore other interesting information-theoretic connections with our framework in Section \ref{section: info theory connections}.
	
	\item Since computing the exact solution to our optimization problem is computationally challenging, we propose instead to greedily select a minimal set of queries by using the \textit{Information Pursuit} (IP) algorithm. IP sequentially selects queries in order of maximum information gain until enough evidence has been gathered, from the query answers, to predict $Y$. This sequence of query-answers serve as the \textit{explanation} for predicting $Y$ from $X$. 
	\item We provide
	sufficient conditions on $Q$ and the joint distribution $p(X, Y)$
	under which the IP strategy comes within $1$ query of the optimal solution.
	(Section \ref{subsection: Approximation guarantees for Information Pursuit}). 
	
	\item Apart from our
	theoretical contributions, we also provide a practical algorithm to
	carry out IP for any task and query set. The difficulty
	of its implementation depends on the structure of the joint
	distribution $p(Q(X),Y)$. We posit a tractable graphical model for
	$p(Q(X),Y)$ and learn the required distributions using Variational
	Autoencoders (VAEs). We then use the Unadjusted Langevin Algorithm
	(ULA) to generate samples required for carrying out IP. 
	
	\item Finally, we demonstrate the utility of our
	framework on vision and NLP tasks (Section \ref{section: Experiments}). In binary images with small patch queries, IP finds succinct explanations whose predictive performance is competitive with state-of-the-art. For example, MNIST requires just about five $3 \times 3$ patch queries on average to decide the digit label. On the CUB-200 dataset, a bird species identification dataset, we use concept-based queries and show how IP explanations can provide insights even to non-experts who might not be able to identify the bird species but can easily understand the concepts IP discovers about the bird leading to its final decision. 
	
	
	%\rene{A concluding sentence about what IP does for these datasets would be good.}
\end{itemize}  



% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.
% However, the Computer Society has been known to put floats at the bottom.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
	%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
	%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.
